Symbolic Autoencoding for Self-Supervised Sequence Learning

Traditional language models, adept at next-token prediction in text sequences, often struggle with transduction tasks between distinct symbolic systems, particularly when parallel data is scarce. Addressing this issue, we introduce \textit{symbolic autoencoding} ($\Sigma$AE), a self-supervised framework that harnesses the power of abundant unparallel data alongside limited parallel data. $\Sigma$AE connects two generative models via a discrete bottleneck layer and is optimized end-to-end by minimizing reconstruction loss (simultaneously with supervised loss for the parallel data), such that the sequence generated by the discrete bottleneck can be read out as the transduced input sequence. We also develop gradient-based methods allowing for efficient self-supervised sequence learning despite the discreteness of the bottleneck. Our results demonstrate that $\Sigma$AE significantly enhances performance on transduction tasks, even with minimal parallel data, offering a promising solution for weakly supervised learning scenarios.

==> figures/discrete-layer-tex.tex <==
\begin{tikzpicture}
    % Define the style for the blocks
    \tikzstyle{block} = [rectangle, draw, text centered, minimum height=2em]
  
    % Nodes for W_o, W_e, and W_d
    \node[block, fill=gray!30] (Wo) at (0,0) {\( W_o \)};
    \node[block, fill=gray!30] (We) at (4,0) {\( W_e \)};
    \node[block, fill=gray!30] (Wd) at (6,-2) {\( W_d \)};
  
    % Stack s_1 to s_N
    \node[block, fill=black!20] (s1) at (2,1) {\( s_1 \)};
    \node[block, fill=black!20] (s2) at (2,0) {\( s_2 \)};
    \node[block, fill=black!20] (sN) at (2,-2) {\( s_N \)};
  
    % Ellipsis for continuation
    \node at (2,-1) {\(\vdots\)};
  
    % Dummy nodes for the stack
    \node (top) at (2,1.5) {}; % Invisible node at the top of the stack
    \node (bottom) at (2,-2.5) {}; % Invisible node at the bottom of the stack
  
    % Connect the nodes
    \draw (top) -- (s1);
    \draw (s1) -- (s2);
    \draw (s2) -- (2,-0.5); % Connection to ellipsis
    \draw (2,-1.5) -- (sN); % Connection from ellipsis
    \draw (sN) -- (bottom);
\end{tikzpicture}

==> figures/results_gumbel.tex <==
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{plots/gumbel_autoreg_hidden_layer_acc_z.png}
  \caption{Gumbel, autoreg\_hidden\_layer\_acc\_z}
  \label{fig:gumbel_autoreg_hidden_layer_acc_z}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{plots/gumbel_autoreg_hidden_layer_sentence_acc_z.png}
  \caption{Gumbel, autoreg\_hidden\_layer\_acc\_z}
  \label{fig:gumbel_autoreg_hidden_layer_sentence_acc_z}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{plots/gumbel_autoreg_acc_z.png}
  \caption{Gumbel, autoreg\_hidden\_layer\_sentence\_acc\_z}
  \label{fig:gumbel_autoreg_acc_z}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{plots/gumbel_autoreg_sentence_acc_z.png}
  \caption{Gumbel, autoreg\_hidden\_layer\_acc\_z}
  \label{fig:gumbel_autoreg_sentence_acc_z}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{plots/gumbel_teacherforced_acc_x.png}
  \caption{Gumbel, teacherforced\_acc\_x}
  \label{fig:gumbel_teacherforced_acc_x}
\end{figure}

==> figures/results_softmax.tex <==
% \begin{figure}
%   \centering
%   \includegraphics[width=1.0\linewidth]{plots/softmax_autoreg_hidden_layer_acc_z.png}
%   \caption{Softmax, autoreg\_hidden\_layer\_acc\_z}
%   \label{fig:softmax_autoreg_hidden_layer_acc_z}
% \end{figure}
% \begin{figure}
%   \centering
%   \includegraphics[width=1.0\linewidth]{plots/softmax_autoreg_hidden_layer_sentence_acc_z.png}
%   \caption{Softmax, autoreg\_hidden\_layer\_acc\_z}
%   \label{fig:softmax_autoreg_hidden_layer_sentence_acc_z}
% \end{figure}
% \begin{figure}
%   \centering
%   \includegraphics[width=1.0\linewidth]{plots/softmax_autoreg_acc_z.png}
%   \caption{Softmax, autoreg\_hidden\_layer\_sentence\_acc\_z}
%   \label{fig:softmax_autoreg_acc_z}
% \end{figure}
% \begin{figure}
%   \centering
%   \includegraphics[width=1.0\linewidth]{plots/softmax_autoreg_sentence_acc_z.png}
%   \caption{Softmax, autoreg\_hidden\_layer\_acc\_z}
%   \label{fig:softmax_autoreg_sentence_acc_z}
% \end{figure}
% \begin{figure}
%   \centering
%   \includegraphics[width=1.0\linewidth]{plots/softmax_teacherforced_acc_x.png}
%   \caption{Softmax, teacherforced\_acc\_x}
%   \label{fig:softmax_teacherforced_acc_x}
% \end{figure}

==> figures/results_vqvae.tex <==
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{plots/vqvae_autoreg_hidden_layer_acc_z.png}
  \caption{VQ-VAE, autoreg\_hidden\_layer\_acc\_z}
  \label{fig:vqvae_autoreg_hidden_layer_acc_z}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{plots/vqvae_autoreg_hidden_layer_sentence_acc_z.png}
  \caption{VQ-VAE, autoreg\_hidden\_layer\_acc\_z}
  \label{fig:vqvae_autoreg_hidden_layer_sentence_acc_z}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{plots/vqvae_autoreg_acc_z.png}
  \caption{VQ-VAE, autoreg\_hidden\_layer\_sentence\_acc\_z}
  \label{fig:vqvae_autoreg_acc_z}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{plots/vqvae_autoreg_sentence_acc_z.png}
  \caption{VQ-VAE, autoreg\_hidden\_layer\_acc\_z}
  \label{fig:vqvae_autoreg_sentence_acc_z}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{plots/vqvae_teacherforced_acc_x.png}
  \caption{VQ-VAE, teacherforced\_acc\_x}
  \label{fig:vqvae_teacherforced_acc_x}
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/02_related_work.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{self supervised discrete sequence learning}

% In \cite{seq3}, the authors connect two encoder-decoder models with the middle layer serving as a hidden sequence. Training occurs end-to-end using a reconstruction loss, resulting in unsupervised sentence compression in the middle layer. Notably, a language model prior loss, derived from the output of a language model, contributes to indirect supervision. Additionally, a topic loss guides the hidden sequence to be proximate to the input.

% \masani{Also they do soft quantization and soft gumbel with straight through estimator (you should go to the code to see it, maybe they actually change it when running the code tho ...). (I don't understand why they call it a straight through when there is no actual discrete sequence in the forward pass.)}
% \masani{should we say that All the losses in our method are simple negative log likelihoods, and we do not use any language models. the point is training smaller models faster in the first place, no?}

Our work intersects with several key studies in unsupervised and weakly supervised learning through discrete representations. In \cite{seq3}, two encoder-decoder models are connected via a hidden sequence layer, utilizing reconstruction loss and language model prior loss for unsupervised sentence compression. \cite{discreteae_bengio} explore semantic hashing \cite{semantichashing} and Gumbel softmax  \cite{gumbel} for creating interpretable, discrete encodings. Similar approaches to discretization, including the use of continuous paths alongside discrete ones, are examined in \cite{somvae}, reflecting the challenges of training with discrete bottlenecks. 
Semi-supervised auto-encoding has been also studied in \cite{semisup_with_gen_kingma}, where the authors treat the classification label as a categorical hidden variable.
Many previous works have studied discretization of elements and representations in neural network \cite{discrete_communication_liu, dvnc_liu, codebook_features_tamkin, backprop_spigot}. 
Our approach stands apart from previous works by (i) employing straightforward negative log-likelihood loss for efficient reconstruction without relying on auxiliary losses, (ii) enabling discretization across sequences of variable lengths, (iii) uniquely blending both unsupervised and supervised data for training, and (iv) integrating sequence models as building blocks for creating sequential autoencoders.

% Our work is closely related to \cite{discreteae_bengio}, where the authors use semantic hashing from \cite{semantichashing} and Gumbel soft-max \cite{gumbel} for discretization, to augment the information from the input sequence to a decoder. Their work achieves interpretable discrete encodings of input sequences. However, their introduced framework accomodates only a fixed length, non-autoregressive function of the input sequence, and the discrete sequence is learned only in an unsupervised manner, not allowing the use of weak supervision for training the discrete representations.
% In \cite{somvae} the authors train a discrete representation similarly, by constructing a continuous path as well as the discrete path for information flow. The continous representations randomly substitute the discrete by a certain probability. Similarly, in \cite{discreteae_bengio}
% Overall our paradigm stands apart from the above as (i) we do not use any losses except simple negative log likelihood in next token prediction or reconstruction (ii) we are not bounded to unsupervised data and can incorporate supervised, parallel data in our training.

 % Related to latter, Semi-supervised auto-encoding has been also studied in \cite{semisup_with_gen_kingma}, where the authors treat the classification label as a categorical hidden variable that is observed when supervised batch is provided, and otherwise unobserved.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Backpropagating through Discrete choice}
% The Vector quantization in \ref{sec:framework_vq} uses the same quantization as \cite{vqvae}
% A large body of works have studied discretization of representations in neural network.
% The idea of quantization with codebooks have been studied in \cite{discrete_communication_liu, dvnc_liu, codebook_features_tamkin, backprop_spigot}. 

% Training with discrete bottlenecks can be difficult even if the representations are not auto-regressively generated. In \cite{somvae} authors alternate between passing a discrete representation or a continuous one in the forward pass, and in \cite{discreteae_bengio} authors start the training with 10000 iterations of continuous representation, and then switch on the discretizer. 
% \cite{backprop_spigot} introduces structured projection of intermediate gradients (SPIGOT), 

% \cite{discrete_communication_liu}: dynamically varying tightness (codebook size) in discrete layer bottlenecks can 
% improve model performance on visual reasoning and reinforcement learning tasks with heterogeneity in representations.

% \cite{dvnc_liu}: restricting the transmitted information among components to discrete representations. 
% try discretiizng an elements in three models. they put the discretization on top of attentiuon layer, so the whole layer
% ends up being still continous through values and it's just so weird. the overall idea is cool. it gets weird in a span of 
% 2 paragraphs all of a sudden.

% \cite{codebook_features_tamkin}: the authors identify codes in Transformer language models representing diverse, 
% disentangled concepts and finds that they can guide the model to generate different topics by activating the 
% appropriate codes during inference, and appears to be a promising unit of analysis and control for neural networks and interpretability.

% \cite{crossmodal_discrete_liu}: a Cross-Modal Code Matching objective that forces the representations from different 
% views (modalities) to have a similar distribution over the discrete embedding space such that cross-modal 
% objects/actions localization can be performed without direct supervision.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{In context learning with Large language models}
% In the same nature of our weak supervision task \ref{sec:framework_scheduling}, recent work on prompting techniques for large language models has discovered that these models can achieve a high performance in a variety of these diagnostic tasks with only a few examples. \cite{least_to_most_zhou, compositional_semantic_parsing_zhou}. 

% recent work \cite{least_to_most_zhou} found that least-to-most prompting shows a lot of
% potential for adapting LLMs for compositional generalization, achieving 99.7\% accuracy on SCAN

% in \cite{compositional_semantic_parsing_zhou} based on least-to-most prompting: it decomposes the
% problem using prompting-based syntactic parsing, then uses this decomposition to
% select appropriate exemplars and to sequentially generate the semantic parse. This
% method allows us to set a new state of the art for CFQ while requiring only 1\%
% of the training data used by traditional approaches.

% We evaluate our approach on two realistic benchmarks that, like SCAN, are designed to measure
% compositional generalization: CFQ \cite{cfq} and COGS \cite{cogs}. On
% CFQ, our best performing method outperforms previous fully supervised finetuning approaches and
% achieves a new state-of-the-art accuracy of 95\% (averaged across MCD splits) and thereby reduced
% the error rate by about 45\% compared to the previous best result while using about 1\% of the training
% data as candidates for exemplars. On COGS, our approach scores an accuracy of 99.2\% when
% evaluated on the generalization test set, comparable with strong baselines. We also demonstrate
% robustness of our approach to exemplar pool size, and when using less than 0.1\% of the training data
% as exemplars, dynamic least-to-most prompting is still competitive with previous approaches.

% Tough baseline but we can compare, we are not afraid are we.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Deep Semi-Supervised Learning}

% In \cite{semisup_with_gen_kingma} the authors introduce a semi-supervised learning approach using deep generative models,
% departing from auto-encoding to learn a generative function for robust representation, with optimization challenges 
% stemming from the need for sampling in loss and gradient minimization. The problem they are solving is similar to our 
% weak supervision task, though they take the classification label as a categorical hidden variable, 
% that is observed sometimes (when supervised batch is provided, and otherwise unobserved).

% comments
% maxime: 

==> tables/results_tables_gumbel_std.tex <==
\begin{table}
  \centering
  \caption{Gumbel DB -- Autoregressive Z TA}
  \label{table:gumbel_validation_hidden_layer_acc}
    % \resizebox{\imagewidth}{!}{
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.75$\pm$0.00} & \multicolumn{1}{c}{0.89$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.76$\pm$0.01} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.80$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.79$\pm$0.00} & \multicolumn{1}{c}{0.90$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.16$\pm$0.00} & \multicolumn{1}{c}{0.25$\pm$0.00} & \multicolumn{1}{c}{0.70$\pm$0.00} & \multicolumn{1}{c}{0.82$\pm$0.00} & \multicolumn{1}{c}{0.89$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.25$\pm$0.00} & \multicolumn{1}{c}{0.66$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.44$\pm$0.00} & \multicolumn{1}{c}{0.62$\pm$0.00} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.56$\pm$0.00} & \multicolumn{1}{c}{0.64$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.74$\pm$0.01} & \multicolumn{1}{c}{0.80$\pm$0.01} & \multicolumn{1}{c}{0.84$\pm$0.01} & \multicolumn{1}{c}{0.85$\pm$0.01} & \multicolumn{1}{c}{0.86$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.76$\pm$0.01} & \multicolumn{1}{c}{0.79$\pm$0.00} & \multicolumn{1}{c}{0.82$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.78$\pm$0.01} & \multicolumn{1}{c}{0.81$\pm$0.01} & \multicolumn{1}{c}{0.84$\pm$0.01} & \multicolumn{1}{c}{0.84$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.75$\pm$0.01} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.01} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.52$\pm$0.00} & \multicolumn{1}{c}{0.57$\pm$0.00} & \multicolumn{1}{c}{0.63$\pm$0.00} & \multicolumn{1}{c}{0.65$\pm$0.00} & \multicolumn{1}{c}{0.65$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.56$\pm$0.00} & \multicolumn{1}{c}{0.62$\pm$0.00} & \multicolumn{1}{c}{0.65$\pm$0.00} & \multicolumn{1}{c}{0.69$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.55$\pm$0.00} & \multicolumn{1}{c}{0.61$\pm$0.00} & \multicolumn{1}{c}{0.65$\pm$0.00} & \multicolumn{1}{c}{0.68$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.60$\pm$0.00} & \multicolumn{1}{c}{0.66$\pm$0.00} & \multicolumn{1}{c}{0.68$\pm$0.00} & \multicolumn{1}{c}{0.71$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}

\begin{table}
  \centering
  \caption{Gumbel DB -- Autoregressive Z SA}
  \label{table:gumbel_validation_hidden_layer_sentence_acc}
    % \resizebox{\imagewidth}{!}{
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.13$\pm$0.00} & \multicolumn{1}{c}{0.46$\pm$0.01} & \multicolumn{1}{c}{0.79$\pm$0.01} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.89$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.22$\pm$0.01} & \multicolumn{1}{c}{0.48$\pm$0.01} & \multicolumn{1}{c}{0.78$\pm$0.01} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.23$\pm$0.01} & \multicolumn{1}{c}{0.56$\pm$0.01} & \multicolumn{1}{c}{0.80$\pm$0.01} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.21$\pm$0.01} & \multicolumn{1}{c}{0.55$\pm$0.01} & \multicolumn{1}{c}{0.81$\pm$0.01} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.01$\pm$0.00} & \multicolumn{1}{c}{0.08$\pm$0.00} & \multicolumn{1}{c}{0.62$\pm$0.00} & \multicolumn{1}{c}{0.76$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.06$\pm$0.00} & \multicolumn{1}{c}{0.57$\pm$0.00} & \multicolumn{1}{c}{0.74$\pm$0.00} & \multicolumn{1}{c}{0.80$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.26$\pm$0.00} & \multicolumn{1}{c}{0.51$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.45$\pm$0.00} & \multicolumn{1}{c}{0.55$\pm$0.00} & \multicolumn{1}{c}{0.75$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.30$\pm$0.00} & \multicolumn{1}{c}{0.48$\pm$0.01} & \multicolumn{1}{c}{0.62$\pm$0.01} & \multicolumn{1}{c}{0.70$\pm$0.01} & \multicolumn{1}{c}{0.73$\pm$0.01} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.41$\pm$0.01} & \multicolumn{1}{c}{0.56$\pm$0.01} & \multicolumn{1}{c}{0.64$\pm$0.01} & \multicolumn{1}{c}{0.68$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.38$\pm$0.01} & \multicolumn{1}{c}{0.53$\pm$0.01} & \multicolumn{1}{c}{0.63$\pm$0.01} & \multicolumn{1}{c}{0.66$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.32$\pm$0.01} & \multicolumn{1}{c}{0.53$\pm$0.01} & \multicolumn{1}{c}{0.63$\pm$0.01} & \multicolumn{1}{c}{0.66$\pm$0.01} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.14$\pm$0.00} & \multicolumn{1}{c}{0.23$\pm$0.00} & \multicolumn{1}{c}{0.30$\pm$0.00} & \multicolumn{1}{c}{0.33$\pm$0.00} & \multicolumn{1}{c}{0.34$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.21$\pm$0.00} & \multicolumn{1}{c}{0.29$\pm$0.00} & \multicolumn{1}{c}{0.34$\pm$0.00} & \multicolumn{1}{c}{0.40$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.21$\pm$0.00} & \multicolumn{1}{c}{0.29$\pm$0.00} & \multicolumn{1}{c}{0.35$\pm$0.00} & \multicolumn{1}{c}{0.39$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.29$\pm$0.00} & \multicolumn{1}{c}{0.37$\pm$0.00} & \multicolumn{1}{c}{0.41$\pm$0.00} & \multicolumn{1}{c}{0.45$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}

% ###############################################################################################
% Results on X


\begin{table}
  \centering
  \caption{Gumbel DB -- Reconstruction Z TA}
  \label{table:gumbel_test_acc_autoreg_z}
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.74$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.90$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{0.90$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.33$\pm$0.00} & \multicolumn{1}{c}{0.46$\pm$0.00} & \multicolumn{1}{c}{0.70$\pm$0.00} & \multicolumn{1}{c}{0.75$\pm$0.00} & \multicolumn{1}{c}{0.79$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.32$\pm$0.00} & \multicolumn{1}{c}{0.58$\pm$0.00} & \multicolumn{1}{c}{0.73$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.56$\pm$0.00} & \multicolumn{1}{c}{0.63$\pm$0.00} & \multicolumn{1}{c}{0.72$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.57$\pm$0.00} & \multicolumn{1}{c}{0.75$\pm$0.00} & \multicolumn{1}{c}{0.82$\pm$0.00} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.90$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.92$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}

\begin{table}
  \centering
  \caption{Gumbel DB -- Reconstruction Z SA}
  \label{table:gumbel_test_sentence_acc_autoreg_z}
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.05$\pm$0.00} & \multicolumn{1}{c}{0.08$\pm$0.00} & \multicolumn{1}{c}{0.17$\pm$0.01} & \multicolumn{1}{c}{0.27$\pm$0.01} & \multicolumn{1}{c}{0.30$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.60$\pm$0.01} & \multicolumn{1}{c}{0.43$\pm$0.01} & \multicolumn{1}{c}{0.54$\pm$0.01} & \multicolumn{1}{c}{0.54$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.65$\pm$0.00} & \multicolumn{1}{c}{0.71$\pm$0.01} & \multicolumn{1}{c}{0.68$\pm$0.01} & \multicolumn{1}{c}{0.62$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.11$\pm$0.00} & \multicolumn{1}{c}{0.18$\pm$0.01} & \multicolumn{1}{c}{0.39$\pm$0.01} & \multicolumn{1}{c}{0.55$\pm$0.01} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.01$\pm$0.00} & \multicolumn{1}{c}{0.06$\pm$0.00} & \multicolumn{1}{c}{0.20$\pm$0.00} & \multicolumn{1}{c}{0.25$\pm$0.00} & \multicolumn{1}{c}{0.21$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.01$\pm$0.00} & \multicolumn{1}{c}{0.11$\pm$0.00} & \multicolumn{1}{c}{0.19$\pm$0.00} & \multicolumn{1}{c}{0.38$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.07$\pm$0.00} & \multicolumn{1}{c}{0.11$\pm$0.00} & \multicolumn{1}{c}{0.15$\pm$0.00} & \multicolumn{1}{c}{0.25$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.05$\pm$0.00} & \multicolumn{1}{c}{0.21$\pm$0.00} & \multicolumn{1}{c}{0.32$\pm$0.00} & \multicolumn{1}{c}{0.42$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
 \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.02$\pm$0.00} & \multicolumn{1}{c}{0.02$\pm$0.00} & \multicolumn{1}{c}{0.20$\pm$0.01} & \multicolumn{1}{c}{0.27$\pm$0.01} & \multicolumn{1}{c}{0.34$\pm$0.01} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.29$\pm$0.01} & \multicolumn{1}{c}{0.48$\pm$0.01} & \multicolumn{1}{c}{0.59$\pm$0.01} & \multicolumn{1}{c}{0.61$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.24$\pm$0.01} & \multicolumn{1}{c}{0.42$\pm$0.01} & \multicolumn{1}{c}{0.56$\pm$0.01} & \multicolumn{1}{c}{0.60$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.30$\pm$0.01} & \multicolumn{1}{c}{0.46$\pm$0.01} & \multicolumn{1}{c}{0.59$\pm$0.01} & \multicolumn{1}{c}{0.63$\pm$0.01} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.05$\pm$0.00} & \multicolumn{1}{c}{0.10$\pm$0.00} & \multicolumn{1}{c}{0.17$\pm$0.00} & \multicolumn{1}{c}{0.21$\pm$0.00} & \multicolumn{1}{c}{0.21$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.10$\pm$0.00} & \multicolumn{1}{c}{0.14$\pm$0.00} & \multicolumn{1}{c}{0.21$\pm$0.00} & \multicolumn{1}{c}{0.25$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.07$\pm$0.00} & \multicolumn{1}{c}{0.13$\pm$0.00} & \multicolumn{1}{c}{0.19$\pm$0.00} & \multicolumn{1}{c}{0.27$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.26$\pm$0.00} & \multicolumn{1}{c}{0.27$\pm$0.00} & \multicolumn{1}{c}{0.31$\pm$0.00} & \multicolumn{1}{c}{0.34$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}


\begin{table}
  \centering
  \caption{Gumbel DB -- Teacher-forced X TA}
  \label{table:gumbel_test_acc_teacher_forced_x}
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.66$\pm$0.00} & \multicolumn{1}{c}{0.76$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.60$\pm$0.00} & \multicolumn{1}{c}{0.70$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.40$\pm$0.00} & \multicolumn{1}{c}{0.63$\pm$0.00} & \multicolumn{1}{c}{0.76$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.36$\pm$0.00} & \multicolumn{1}{c}{0.64$\pm$0.00} & \multicolumn{1}{c}{0.62$\pm$0.00} & \multicolumn{1}{c}{0.76$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.39$\pm$0.00} & \multicolumn{1}{c}{0.48$\pm$0.00} & \multicolumn{1}{c}{0.51$\pm$0.00} & \multicolumn{1}{c}{0.55$\pm$0.00} & \multicolumn{1}{c}{0.57$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.38$\pm$0.00} & \multicolumn{1}{c}{0.49$\pm$0.00} & \multicolumn{1}{c}{0.55$\pm$0.00} & \multicolumn{1}{c}{0.58$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.45$\pm$0.00} & \multicolumn{1}{c}{0.50$\pm$0.00} & \multicolumn{1}{c}{0.52$\pm$0.00} & \multicolumn{1}{c}{0.56$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.43$\pm$0.00} & \multicolumn{1}{c}{0.53$\pm$0.00} & \multicolumn{1}{c}{0.55$\pm$0.00} & \multicolumn{1}{c}{0.57$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.71$\pm$0.00} & \multicolumn{1}{c}{0.77$\pm$0.00} & \multicolumn{1}{c}{0.80$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} & \multicolumn{1}{c}{0.85$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.75$\pm$0.00} & \multicolumn{1}{c}{0.79$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.72$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.69$\pm$0.00} & \multicolumn{1}{c}{0.77$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}



% \begin{table}
%   \centering
%   \caption{Discretizer: Gumbel. ZXZ only, Test autoregressive accuracy $Z$ (top) and sentence accuracy $Z$ (bottom) with 0.01 of data.}
%   \label{table:gumbel_zxz_only_validation_acc}
%     \resizebox{\imagewidth}{!}{
%         \begin{tabular}{ccccc}
%         \\
%           \hline
%           \multicolumn{1}{c}{SCAN}
%         & \multicolumn{1}{c}{SFST}  & \multicolumn{1}{c}{PCFG}   & \multicolumn{1}{c}{COGS} & CFQ \\
%           \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.98$\pm0.00$} \\
%           \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.41$\pm0.00$}
%           \\ \hline
%         \end{tabular}
%       }
% \end{table}


% % \end{document}

==> tables/results_tables_softmax_std.tex <==
\begin{table}
  \centering
  \caption{Softmax DB -- Autoregressive Z TA}
  \label{table:softmax_validation_hidden_layer_acc}
    % \resizebox{\imagewidth}{!}{
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.92$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.76$\pm$0.00} & \multicolumn{1}{c}{0.89$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00}  & \multicolumn{1}{c}{---}\\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00}  & \multicolumn{1}{c}{---}\\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.79$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00}  & \multicolumn{1}{c}{---}\\  \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.17$\pm$0.00} & \multicolumn{1}{c}{0.30$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.56$\pm$0.00} & \multicolumn{1}{c}{0.77$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00}  & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.47$\pm$0.00} & \multicolumn{1}{c}{0.73$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00}  & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.58$\pm$0.00} & \multicolumn{1}{c}{0.82$\pm$0.00} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00}  & \multicolumn{1}{c}{---} \\  \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00}  & \multicolumn{1}{c}{---}\\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00}  & \multicolumn{1}{c}{---}\\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00}  & \multicolumn{1}{c}{---} \\  \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.62$\pm$0.00} & \multicolumn{1}{c}{0.70$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.82$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.69$\pm$0.00} & \multicolumn{1}{c}{0.75$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00}  & \multicolumn{1}{c}{---}\\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.73$\pm$0.00} & \multicolumn{1}{c}{0.80$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00}  & \multicolumn{1}{c}{---}\\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.71$\pm$0.00} & \multicolumn{1}{c}{0.79$\pm$0.00} & \multicolumn{1}{c}{0.82$\pm$0.00} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}

\begin{table}
  \centering
  \caption{Softmax DB -- Autoregressive Z SA}
  \label{table:softmax_validation_hidden_layer_sentence_acc}
    % \resizebox{\imagewidth}{!}{
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.18$\pm$0.01} & \multicolumn{1}{c}{0.52$\pm$0.01} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.24$\pm$0.01} & \multicolumn{1}{c}{0.50$\pm$0.01} & \multicolumn{1}{c}{0.87$\pm$0.01} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.29$\pm$0.01} & \multicolumn{1}{c}{0.71$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.25$\pm$0.00} & \multicolumn{1}{c}{0.61$\pm$0.01} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\ 
        %   \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.01$\pm$0.00} & \multicolumn{1}{c}{0.11$\pm$0.00} & \multicolumn{1}{c}{0.75$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.45$\pm$0.00} & \multicolumn{1}{c}{0.73$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.92$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.32$\pm$0.00} & \multicolumn{1}{c}{0.70$\pm$0.00} & \multicolumn{1}{c}{0.92$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.47$\pm$0.01} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.48$\pm$0.01} & \multicolumn{1}{c}{0.71$\pm$0.01} & \multicolumn{1}{c}{0.89$\pm$0.01} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.63$\pm$0.01} & \multicolumn{1}{c}{0.82$\pm$0.01} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
          \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.60$\pm0.00$} & \multicolumn{1}{c}{0.83$\pm0.00$} & 0.94$\pm0.00$ & \multicolumn{1}{c}{0.97$\pm0.00$}  & \multicolumn{1}{c}{---} \\ 
          \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.66$\pm$0.01} & \multicolumn{1}{c}{0.84$\pm$0.01} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---}  \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.25$\pm$0.00} & \multicolumn{1}{c}{0.40$\pm$0.00} & \multicolumn{1}{c}{0.53$\pm$0.00} & \multicolumn{1}{c}{0.61$\pm$0.00} & \multicolumn{1}{c}{0.69$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.43$\pm$0.00} & \multicolumn{1}{c}{0.50$\pm$0.00} & \multicolumn{1}{c}{0.65$\pm$0.00} & \multicolumn{1}{c}{0.73$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.49$\pm$0.00} & \multicolumn{1}{c}{0.59$\pm$0.00} & \multicolumn{1}{c}{0.66$\pm$0.00} & \multicolumn{1}{c}{0.73$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.47$\pm$0.00} & \multicolumn{1}{c}{0.60$\pm$0.00} & \multicolumn{1}{c}{0.64$\pm$0.00} & \multicolumn{1}{c}{0.69$\pm$0.00} & \multicolumn{1}{c}{---} \\  \hline
        \end{tabular}
      }
\end{table}



% ###############################################################################################
% Results on X

\begin{table}
  \centering
  \caption{Softmax DB -- Reconstruction Z TA}
  \label{table:softmax_test_acc_autoreg_z}
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.74$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.89$\pm$0.00} & \multicolumn{1}{c}{0.92$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.37$\pm$0.00} & \multicolumn{1}{c}{0.50$\pm$0.00} & \multicolumn{1}{c}{0.74$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.71$\pm$0.00} & \multicolumn{1}{c}{0.80$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.68$\pm$0.00} & \multicolumn{1}{c}{0.75$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.89$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.76$\pm$0.00} & \multicolumn{1}{c}{0.79$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.92$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}

\begin{table}
  \centering
  \caption{Softmax DB -- Reconstruction Z SA}
  \label{table:softmax_test_sentence_acc_autoreg_z}
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.05$\pm$0.00} & \multicolumn{1}{c}{0.11$\pm$0.00} & \multicolumn{1}{c}{0.24$\pm$0.00} & \multicolumn{1}{c}{0.28$\pm$0.01} & \multicolumn{1}{c}{0.46$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.82$\pm$0.01} & \multicolumn{1}{c}{0.76$\pm$0.01} & \multicolumn{1}{c}{0.72$\pm$0.01} & \multicolumn{1}{c}{0.65$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.90$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.01} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.66$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{0.18$\pm$0.01} & \multicolumn{1}{c}{0.41$\pm$0.01} & \multicolumn{1}{c}{0.66$\pm$0.01} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.01$\pm$0.00} & \multicolumn{1}{c}{0.09$\pm$0.00} & \multicolumn{1}{c}{0.20$\pm$0.00} & \multicolumn{1}{c}{0.28$\pm$0.00} & \multicolumn{1}{c}{0.35$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.21$\pm$0.00} & \multicolumn{1}{c}{0.29$\pm$0.00} & \multicolumn{1}{c}{0.44$\pm$0.00} & \multicolumn{1}{c}{0.63$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.15$\pm$0.00} & \multicolumn{1}{c}{0.22$\pm$0.00} & \multicolumn{1}{c}{0.33$\pm$0.01} & \multicolumn{1}{c}{0.47$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.19$\pm$0.00} & \multicolumn{1}{c}{0.26$\pm$0.00} & \multicolumn{1}{c}{0.44$\pm$0.01} & \multicolumn{1}{c}{0.41$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.02$\pm$0.00} & \multicolumn{1}{c}{0.04$\pm$0.00} & \multicolumn{1}{c}{0.35$\pm$0.01} & \multicolumn{1}{c}{0.48$\pm$0.01} & \multicolumn{1}{c}{0.57$\pm$0.01} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.51$\pm$0.01} & \multicolumn{1}{c}{0.76$\pm$0.01} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.55$\pm$0.00} & \multicolumn{1}{c}{0.48$\pm$0.00} & \multicolumn{1}{c}{0.68$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.75$\pm$0.01} & \multicolumn{1}{c}{0.81$\pm$0.01} & \multicolumn{1}{c}{0.90$\pm$0.01} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.11$\pm$0.00} & \multicolumn{1}{c}{0.23$\pm$0.00} & \multicolumn{1}{c}{0.36$\pm$0.00} & \multicolumn{1}{c}{0.48$\pm$0.00} & \multicolumn{1}{c}{0.53$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.29$\pm$0.00} & \multicolumn{1}{c}{0.36$\pm$0.00} & \multicolumn{1}{c}{0.50$\pm$0.00} & \multicolumn{1}{c}{0.61$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.36$\pm$0.00} & \multicolumn{1}{c}{0.44$\pm$0.00} & \multicolumn{1}{c}{0.54$\pm$0.00} & \multicolumn{1}{c}{0.62$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.40$\pm$0.00} & \multicolumn{1}{c}{0.51$\pm$0.00} & \multicolumn{1}{c}{0.52$\pm$0.00} & \multicolumn{1}{c}{0.60$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}

\begin{table}
  \centering
  \caption{Softmax DB -- Teacher-forced X TA}
  \label{table:softmax_test_acc_teacher_forced_x}
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.66$\pm$0.00} & \multicolumn{1}{c}{0.77$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.57$\pm$0.00} & \multicolumn{1}{c}{0.66$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.39$\pm$0.00} & \multicolumn{1}{c}{0.58$\pm$0.00} & \multicolumn{1}{c}{0.70$\pm$0.00} & \multicolumn{1}{c}{0.82$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.50$\pm$0.00} & \multicolumn{1}{c}{0.45$\pm$0.00} & \multicolumn{1}{c}{0.69$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.41$\pm$0.00} & \multicolumn{1}{c}{0.50$\pm$0.00} & \multicolumn{1}{c}{0.53$\pm$0.00} & \multicolumn{1}{c}{0.57$\pm$0.00} & \multicolumn{1}{c}{0.65$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.50$\pm$0.00} & \multicolumn{1}{c}{0.54$\pm$0.00} & \multicolumn{1}{c}{0.57$\pm$0.00} & \multicolumn{1}{c}{0.61$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.47$\pm$0.00} & \multicolumn{1}{c}{0.50$\pm$0.00} & \multicolumn{1}{c}{0.54$\pm$0.00} & \multicolumn{1}{c}{0.57$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.48$\pm$0.00} & \multicolumn{1}{c}{0.50$\pm$0.00} & \multicolumn{1}{c}{0.61$\pm$0.00} & \multicolumn{1}{c}{0.63$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.90$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.74$\pm$0.00} & \multicolumn{1}{c}{0.79$\pm$0.00} & \multicolumn{1}{c}{0.82$\pm$0.00} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.77$\pm$0.00} & \multicolumn{1}{c}{0.80$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.73$\pm$0.00} & \multicolumn{1}{c}{0.80$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.71$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.82$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}

% \begin{table}
%   \centering
%   \caption{Discretizer: Softmax. ZXZ only, Test autoregressive accuracy $Z$ (top) and sentence accuracy $Z$ (bottom) with 0.01 of data.}
%   \label{table:softmax_zxz_only_validation_acc}
%     \resizebox{\imagewidth}{!}{
%         \begin{tabular}{ccccc}
%         \\
%           \hline
%           \multicolumn{1}{c}{SCAN}
%         & \multicolumn{1}{c}{SFST}  & \multicolumn{1}{c}{PCFG}   & \multicolumn{1}{c}{COGS} & CFQ \\
%           \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} \\
%           \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}
%           \\ \hline
%         \end{tabular}
%       }
% \end{table}


% % \end{document}

==> tables/results_tables_vqvae_std.tex <==
\begin{table}
  \centering
  \caption{VQ DB -- Autoregressive Z TA}
  \label{table:vqvae_validation_hidden_layer_acc}
    % \resizebox{\imagewidth}{!}{
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.73$\pm$0.00} & \multicolumn{1}{c}{0.89$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.67$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.75$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.23$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.31$\pm$0.00} & \multicolumn{1}{c}{0.66$\pm$0.00} & \multicolumn{1}{c}{0.90$\pm$0.00} & \multicolumn{1}{c}{0.89$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.41$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.90$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.12$\pm$0.00} & \multicolumn{1}{c}{0.13$\pm$0.00} & \multicolumn{1}{c}{0.13$\pm$0.00} & \multicolumn{1}{c}{0.13$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.86$\pm$0.01} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.92$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.91$\pm$0.01} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.49$\pm$0.00} & \multicolumn{1}{c}{0.77$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.71$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.69$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.44$\pm$0.00} & \multicolumn{1}{c}{0.54$\pm$0.00} & \multicolumn{1}{c}{0.52$\pm$0.00} & \multicolumn{1}{c}{0.61$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}

\begin{table}
  \centering
  \caption{VQ DB -- Autoregressive Z SA}
  \label{table:vqvae_validation_hidden_layer_sentence_acc}
    % \resizebox{\imagewidth}{!}{
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.10$\pm$0.01} & \multicolumn{1}{c}{0.41$\pm$0.01} & \multicolumn{1}{c}{0.85$\pm$0.01} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.12$\pm$0.01} & \multicolumn{1}{c}{0.44$\pm$0.01} & \multicolumn{1}{c}{0.70$\pm$0.01} & \multicolumn{1}{c}{0.87$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.29$\pm$0.00} & \multicolumn{1}{c}{0.64$\pm$0.01} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.15$\pm$0.01} & \multicolumn{1}{c}{0.54$\pm$0.01} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.04$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.14$\pm$0.00} & \multicolumn{1}{c}{0.59$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.89$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.23$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.90$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.47$\pm$0.01} & \multicolumn{1}{c}{0.74$\pm$0.01} & \multicolumn{1}{c}{0.92$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.01} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.51$\pm$0.01} & \multicolumn{1}{c}{0.81$\pm$0.01} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.59$\pm$0.01} & \multicolumn{1}{c}{0.82$\pm$0.01} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.51$\pm$0.01} & \multicolumn{1}{c}{0.63$\pm$0.01} & \multicolumn{1}{c}{0.62$\pm$0.01} & \multicolumn{1}{c}{0.59$\pm$0.01} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.01$\pm$0.00} & \multicolumn{1}{c}{0.53$\pm$0.00} & \multicolumn{1}{c}{0.79$\pm$0.00} & \multicolumn{1}{c}{0.87$\pm$0.00} & \multicolumn{1}{c}{0.25$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.69$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.92$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.41$\pm$0.00} & \multicolumn{1}{c}{0.66$\pm$0.00} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.01$\pm$0.00} & \multicolumn{1}{c}{0.02$\pm$0.00} & \multicolumn{1}{c}{0.07$\pm$0.00} & \multicolumn{1}{c}{0.05$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}


% ###############################################################################################
% Results on X



\begin{table}
  \centering
  \caption{VQ DB -- Reconstruction Z TA}
  \label{table:vqvae_test_acc_autoreg_z}
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.73$\pm$0.00} & \multicolumn{1}{c}{0.77$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.35$\pm$0.00} & \multicolumn{1}{c}{0.67$\pm$0.00} & \multicolumn{1}{c}{0.77$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.53$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.59$\pm$0.00} & \multicolumn{1}{c}{0.77$\pm$0.00} & \multicolumn{1}{c}{0.91$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.68$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} & \multicolumn{1}{c}{0.89$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.32$\pm$0.00} & \multicolumn{1}{c}{0.38$\pm$0.00} & \multicolumn{1}{c}{0.32$\pm$0.00} & \multicolumn{1}{c}{0.32$\pm$0.00} & \multicolumn{1}{c}{---} \\\hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{1.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.89$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.97$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{0.94$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}

\begin{table}
  \centering
  \caption{VQ DB -- Reconstruction Z SA}
  \label{table:vqvae_test_sentence_acc_autoreg_z}
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.05$\pm$0.00} & \multicolumn{1}{c}{0.12$\pm$0.00} & \multicolumn{1}{c}{0.29$\pm$0.01} & \multicolumn{1}{c}{0.61$\pm$0.01} & \multicolumn{1}{c}{0.91$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.40$\pm$0.01} & \multicolumn{1}{c}{0.38$\pm$0.01} & \multicolumn{1}{c}{0.39$\pm$0.01} & \multicolumn{1}{c}{0.52$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.89$\pm$0.00} & \multicolumn{1}{c}{0.76$\pm$0.00} & \multicolumn{1}{c}{0.71$\pm$0.01} & \multicolumn{1}{c}{0.66$\pm$0.01} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.17$\pm$0.00} & \multicolumn{1}{c}{0.67$\pm$0.00} & \multicolumn{1}{c}{0.90$\pm$0.01} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.02$\pm$0.00} & \multicolumn{1}{c}{0.18$\pm$0.00} & \multicolumn{1}{c}{0.19$\pm$0.00} & \multicolumn{1}{c}{0.25$\pm$0.00} & \multicolumn{1}{c}{0.12$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.10$\pm$0.00} & \multicolumn{1}{c}{0.30$\pm$0.00} & \multicolumn{1}{c}{0.64$\pm$0.00} & \multicolumn{1}{c}{0.75$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.13$\pm$0.00} & \multicolumn{1}{c}{0.33$\pm$0.00} & \multicolumn{1}{c}{0.39$\pm$0.00} & \multicolumn{1}{c}{0.56$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.32$\pm$0.01} & \multicolumn{1}{c}{0.68$\pm$0.01} & \multicolumn{1}{c}{0.78$\pm$0.01} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.39$\pm$0.01} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.41$\pm$0.01} & \multicolumn{1}{c}{0.68$\pm$0.01} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.35$\pm$0.01} & \multicolumn{1}{c}{0.69$\pm$0.01} & \multicolumn{1}{c}{0.88$\pm$0.01} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.44$\pm$0.01} & \multicolumn{1}{c}{0.57$\pm$0.01} & \multicolumn{1}{c}{0.52$\pm$0.01} & \multicolumn{1}{c}{0.53$\pm$0.01} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.01$\pm$0.00} & \multicolumn{1}{c}{0.19$\pm$0.00} & \multicolumn{1}{c}{0.51$\pm$0.00} & \multicolumn{1}{c}{0.52$\pm$0.00} & \multicolumn{1}{c}{0.22$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.27$\pm$0.00} & \multicolumn{1}{c}{0.40$\pm$0.00} & \multicolumn{1}{c}{0.57$\pm$0.00} & \multicolumn{1}{c}{0.67$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.19$\pm$0.00} & \multicolumn{1}{c}{0.41$\pm$0.00} & \multicolumn{1}{c}{0.56$\pm$0.00} & \multicolumn{1}{c}{0.71$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{0.01$\pm$0.00} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{0.00$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}


\begin{table}
  \centering
  \caption{VQ DB -- Teacher-forced X TA}
  \label{table:vqvae_test_acc_teacher_forced_x}
    {
        \begin{tabular}{c ccccc}
          \hline
          \multicolumn{1}{c}{SCAN}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.65$\pm$0.00} & \multicolumn{1}{c}{0.73$\pm$0.00} & \multicolumn{1}{c}{0.81$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.56$\pm$0.00} & \multicolumn{1}{c}{0.67$\pm$0.00} & \multicolumn{1}{c}{0.74$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.41$\pm$0.00} & \multicolumn{1}{c}{0.62$\pm$0.00} & \multicolumn{1}{c}{0.71$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.27$\pm$0.00} & \multicolumn{1}{c}{0.61$\pm$0.00} & \multicolumn{1}{c}{0.57$\pm$0.00} & \multicolumn{1}{c}{0.79$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
        %   \multicolumn{1}{c}{SFST}
        % & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
        %   \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$}  \\
        %   \multirow{1}{*}{Mixed}  & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}  & \multicolumn{1}{c}{---} \\
        %   \multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{PCFG}
        & \multicolumn{1}{c}{$\eta=0.04$}  & \multicolumn{1}{c}{$\eta=0.08$}   & \multicolumn{1}{c}{$\eta=0.16$} & $\eta=0.32$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.32$\pm$0.00} & \multicolumn{1}{c}{0.52$\pm$0.00} & \multicolumn{1}{c}{0.55$\pm$0.00} & \multicolumn{1}{c}{0.58$\pm$0.00} & \multicolumn{1}{c}{0.62$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.43$\pm$0.00} & \multicolumn{1}{c}{0.54$\pm$0.00} & \multicolumn{1}{c}{0.59$\pm$0.00} & \multicolumn{1}{c}{0.65$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.48$\pm$0.00} & \multicolumn{1}{c}{0.53$\pm$0.00} & \multicolumn{1}{c}{0.55$\pm$0.00} & \multicolumn{1}{c}{0.58$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.33$\pm$0.00} & \multicolumn{1}{c}{0.34$\pm$0.00} & \multicolumn{1}{c}{0.33$\pm$0.00} & \multicolumn{1}{c}{0.33$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{COGS}
        & \multicolumn{1}{c}{$\eta=0.02$}  & \multicolumn{1}{c}{$\eta=0.04$}   & \multicolumn{1}{c}{$\eta=0.08$} & $\eta=0.16$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{0.96$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{0.97$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{0.95$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.85$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.98$\pm$0.00} & \multicolumn{1}{c}{0.99$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.88$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{0.93$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline\hline
          \multicolumn{1}{c}{CFQ}
        & \multicolumn{1}{c}{$\eta=0.01$}  & \multicolumn{1}{c}{$\eta=0.02$}   & \multicolumn{1}{c}{$\eta=0.04$} & $\eta=0.08$ & $\eta=0.99$ \\ \cmidrule(lr){2-6}
          \multirow{1}{*}{Supervised} & \multicolumn{1}{c}{0.60$\pm$0.00} & \multicolumn{1}{c}{0.77$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{0.88$\pm$0.00} \\ 
\multirow{1}{*}{Mixed} & \multicolumn{1}{c}{0.74$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.83$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{s\rightarrow u}$} & \multicolumn{1}{c}{0.68$\pm$0.00} & \multicolumn{1}{c}{0.78$\pm$0.00} & \multicolumn{1}{c}{0.84$\pm$0.00} & \multicolumn{1}{c}{0.86$\pm$0.00} & \multicolumn{1}{c}{---} \\ 
\multirow{1}{*}{Curriculum$^{u\rightarrow s}$} & \multicolumn{1}{c}{0.49$\pm$0.00} & \multicolumn{1}{c}{0.55$\pm$0.00} & \multicolumn{1}{c}{0.53$\pm$0.00} & \multicolumn{1}{c}{0.53$\pm$0.00} & \multicolumn{1}{c}{---} \\ \hline
        \end{tabular}
      }
\end{table}






% \begin{table}
%   \centering
%   \caption{Discretizer: VQ-VAE. ZXZ only, Test autoregressive accuracy $Z$ (top) and sentence accuracy $Z$ (bottom) with 0.01 of data.}
%   \label{table:vqvae_zxz_only_validation_acc}
%     \resizebox{\imagewidth}{!}{
%         \begin{tabular}{ccccc}
%         \\
%           \hline
%           \multicolumn{1}{c}{SCAN}
%         & \multicolumn{1}{c}{SFST}  & \multicolumn{1}{c}{PCFG}   & \multicolumn{1}{c}{COGS} & CFQ \\
%           \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$} \\
%           \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & \multicolumn{1}{c}{0.00$\pm0.00$} & 0.00$\pm0.00$ & \multicolumn{1}{c}{0.00$\pm0.00$}
%           \\ \hline
%         \end{tabular}
%       }
% \end{table}


% % \end{document}
